On Coded Caching Systems with Offline Users

Coded caching is a technique that leverages locally cached contents at the users to reduce the network's peak-time communication load. Coded caching achieves significant performance gains compared to uncoded caching schemes and is thus a promising technique to boost performance in future networks. In the original model introduced by Maddah-Ali and Niesen (MAN), a server stores multiple files and is connected to multiple cache-aided users through an error-free shared link; once the local caches have been filled and all users have sent their demand to the server, the server can start sending coded multicast messages to satisfy all users' demands. A practical limitation of the original MAN model is that it halts if the server does not receive all users' demands, which is the limiting case of asynchronous coded caching when the requests of some users arrive with infinite delay. In this paper we formally define a coded caching system where some users are offline. We propose achievable and converse bounds for this novel setting and show under which conditions they meet, thus providing an optimal solution, and when they are to within a constant multiplicative gap of two. Interestingly, when optimality can be be shown, the optimal load-memory tradeoff only depends on the number active users, and not on the total (active plus offline) number of users.

==> ieeemacro.tex <==


\newcommand{\Bv}{{\mathbf B}}


\newcommand{\CC}{{\mathbb C}}
\newcommand{\PP}{{\mathbb P}}
\newcommand{\RR}{{\mathbb R}}
\newcommand{\QQ}{{\mathbb Q}}
\newcommand{\ZZ}{{\mathbb Z}}
\newcommand{\FF}{{\mathbb F}}
\newcommand{\GG}{{\mathbb G}}
\newcommand{\EE}{{\mathbb E}}
\newcommand{\NN}{{\mathbb N}}
\newcommand{\KK}{{\mathbb K}}


\newcommand{\av}{{\mathbf a}}
\newcommand{\bv}{{\mathbf b}}
\newcommand{\cv}{{\mathbf c}}
\newcommand{\dv}{{\mathbf d}}
\newcommand{\ev}{{\mathbf e}}
\newcommand{\fv}{{\mathbf f}}
\newcommand{\gv}{{\mathbf g}}
\newcommand{\hv}{{\mathbf h}}
\newcommand{\iv}{{\mathbf i}}
\newcommand{\jv}{{\mathbf j}}
\newcommand{\kv}{{\mathbf k}}
\newcommand{\lv}{{\mathbf l}}
\newcommand{\mv}{{\mathbf m}}
\newcommand{\nv}{{\mathbf n}}
\newcommand{\ov}{{\mathbf o}}
\newcommand{\pv}{{\mathbf p}}
\newcommand{\qv}{{\mathbf q}}
\newcommand{\rv}{{\mathbf r}}
\newcommand{\sv}{{\mathbf s}}
\newcommand{\tv}{{\mathbf t}}
\newcommand{\uv}{{\mathbf u}}
\newcommand{\wv}{{\mathbf w}}
\newcommand{\vv}{{\mathbf v}}
\newcommand{\xv}{{\mathbf x}}
\newcommand{\yv}{{\mathbf y}}
\newcommand{\zv}{{\mathbf z}}
\newcommand{\zerov}{{\mathbf 0}}
\newcommand{\onev}{{\mathbf 1}}


\newcommand{\Am}{{\mathbf A}}
\newcommand{\Bm}{{\mathbf B}}
\newcommand{\Cm}{{\mathbf C}}
\newcommand{\Dm}{{\mathbf D}}
\newcommand{\Em}{{\mathbf E}}
\newcommand{\Fm}{{\mathbf F}}
\newcommand{\Gm}{{\mathbf G}}
\newcommand{\Hm}{{\mathbf H}}
\newcommand{\Id}{{\mathbf I}}
\newcommand{\Jm}{{\mathbf J}}
\newcommand{\Km}{{\mathbf K}}
\newcommand{\Lm}{{\mathbf L}}
\newcommand{\Mm}{{\mathbf M}}
\newcommand{\Nm}{{\mathbf N}}
\newcommand{\Om}{{\mathbf O}}
\newcommand{\Pm}{{\mathbf P}}
\newcommand{\Qm}{{\mathbf Q}}
\newcommand{\Rm}{{\mathbf R}}
\newcommand{\Sm}{{\mathbf S}}
\newcommand{\Tm}{{\mathbf T}}
\newcommand{\Um}{{\mathbf U}}
\newcommand{\Wm}{{\mathbf W}}
\newcommand{\Vm}{{\mathbf V}}
\newcommand{\Xm}{{\mathbf X}}
\newcommand{\Ym}{{\mathbf Y}}
\newcommand{\Zm}{{\mathbf Z}}


\newcommand{\Ac}{{\magenta \mathcal A}}
\newcommand{\Bc}{{\mathcal B}}
\newcommand{\Cc}{{\mathcal C}}
\newcommand{\Dc}{{\mathcal D}}
\newcommand{\Ec}{{\mathcal E}}
\newcommand{\Fc}{{\mathcal F}}
\newcommand{\Gc}{{\mathcal G}}
\newcommand{\Hc}{{\mathcal H}}
\newcommand{\Ic}{{\mathcal I}}
\newcommand{\Jc}{{\mathcal J}}
\newcommand{\Kc}{{\mathcal K}}
\newcommand{\Lc}{{\blue \mathcal L}}
\newcommand{\Mc}{{\mathcal M}}
\newcommand{\Nc}{{\mathcal N}}
\newcommand{\Oc}{{\mathcal O}}
\newcommand{\Pc}{{\mathcal P}}
\newcommand{\Qc}{{\mathcal Q}}
\newcommand{\Rc}{{\mathcal R}}
\newcommand{\Sc}{{\mathcal S}}
\newcommand{\Tc}{{\mathcal T}}
\newcommand{\Uc}{{\mathcal U}}
\newcommand{\Wc}{{\mathcal W}}
\newcommand{\Vc}{{\mathcal V}}
\newcommand{\Xc}{{\mathcal X}}
\newcommand{\Yc}{{\mathcal Y}}
\newcommand{\Zc}{{\mathcal Z}}


\newcommand{\alphav}{\hbox{\boldmath$\alpha$}}
\newcommand{\betav}{\hbox{\boldmath$\beta$}}
\newcommand{\gammav}{\hbox{\boldmath$\gamma$}}
\newcommand{\deltav}{\hbox{\boldmath$\delta$}}
\newcommand{\etav}{\hbox{\boldmath$\eta$}}
\newcommand{\lambdav}{\hbox{\boldmath$\lambda$}}
\newcommand{\epsilonv}{\hbox{\boldmath$\epsilon$}}
\newcommand{\nuv}{\hbox{\boldmath$\nu$}}
\newcommand{\muv}{\hbox{\boldmath$\mu$}}
\newcommand{\zetav}{\hbox{\boldmath$\zeta$}}
\newcommand{\phiv}{\hbox{\boldmath$\phi$}}
\newcommand{\psiv}{\hbox{\boldmath$\psi$}}
\newcommand{\thetav}{\hbox{\boldmath$\theta$}}
\newcommand{\tauv}{\hbox{\boldmath$\tau$}}
\newcommand{\omegav}{\hbox{\boldmath$\omega$}}
\newcommand{\xiv}{\hbox{\boldmath$\xi$}}
\newcommand{\sigmav}{\hbox{\boldmath$\sigma$}}
\newcommand{\piv}{\hbox{\boldmath$\pi$}}
\newcommand{\rhov}{\hbox{\boldmath$\rho$}}
\newcommand{\Gammam}{\hbox{\boldmath$\Gamma$}}
\newcommand{\Lambdam}{\hbox{\boldmath$\Lambda$}}
\newcommand{\Deltam}{\hbox{\boldmath$\Delta$}}
\newcommand{\Sigmam}{\hbox{\boldmath$\Sigma$}}
\newcommand{\Phim}{\hbox{\boldmath$\Phi$}}
\newcommand{\Pim}{\hbox{\boldmath$\Pi$}}
\newcommand{\Psim}{\hbox{\boldmath$\Psi$}}
\newcommand{\Thetam}{\hbox{\boldmath$\Theta$}}
\newcommand{\Omegam}{\hbox{\boldmath$\Omega$}}
\newcommand{\Xim}{\hbox{\boldmath$\Xi$}}



\newcommand{\asf}{{\mathsf a}}
\newcommand{\bsf}{{\mathsf b}}
\newcommand{\csf}{{\mathsf c}}
\newcommand{\dsf}{{\mathsf d}}
\newcommand{\esf}{{\mathsf e}}
\newcommand{\fsf}{{\mathsf f}}
\newcommand{\gsf}{{\mathsf g}}
\newcommand{\hsf}{{\mathsf h}}
\newcommand{\isf}{{\mathsf i}}
\newcommand{\jsf}{{\mathsf j}}
\newcommand{\ksf}{{\mathsf k}}
\newcommand{\lsf}{{\mathsf l}}
\newcommand{\msf}{{\mathsf m}}
\newcommand{\nsf}{{\mathsf n}}
\newcommand{\osf}{{\mathsf o}}
\newcommand{\psf}{{\mathsf p}}
\newcommand{\qsf}{{\mathsf q}}
\newcommand{\rsf}{{\mathsf r}}
\newcommand{\ssf}{{\mathsf s}}
\newcommand{\tsf}{{\mathsf t}}
\newcommand{\usf}{{\mathsf u}}
\newcommand{\wsf}{{\mathsf w}}
\newcommand{\vsf}{{\mathsf v}}
\newcommand{\xsf}{{\mathsf x}}
\newcommand{\ysf}{{\mathsf y}}
\newcommand{\zsf}{{\mathsf z}}


\newcommand{\Asf}{{\mathsf A}}
\newcommand{\Bsf}{{\mathsf B}}
\newcommand{\Csf}{{\mathsf C}}
\newcommand{\Dsf}{{\mathsf D}}
\newcommand{\Esf}{{\mathsf E}}
\newcommand{\Fsf}{{\mathsf F}}
\newcommand{\Gsf}{{\mathsf G}}
\newcommand{\Hsf}{{\mathsf H}}
\newcommand{\Isf}{{\mathsf I}}
\newcommand{\Jsf}{{\mathsf J}}
\newcommand{\Ksf}{{\mathsf K}}
\newcommand{\Lsf}{{\mathsf L}}
\newcommand{\Msf}{{\mathsf M}}
\newcommand{\Nsf}{{\mathsf N}}
\newcommand{\Osf}{{\mathsf O}}
\newcommand{\Psf}{{\mathsf P}}
\newcommand{\Qsf}{{\mathsf Q}}
\newcommand{\Rsf}{{\mathsf R}}
\newcommand{\Ssf}{{\mathsf S}}
\newcommand{\Tsf}{{\mathsf T}}
\newcommand{\Usf}{{\mathsf U}}
\newcommand{\Wsf}{{\mathsf W}}
\newcommand{\Vsf}{{\mathsf V}}
\newcommand{\Xsf}{{\mathsf X}}
\newcommand{\Ysf}{{\mathsf Y}}
\newcommand{\Zsf}{{\mathsf Z}}


\newcommand{\sinc}{{\hbox{sinc}}}
\newcommand{\diag}{{\hbox{diag}}}
\renewcommand{\det}{{\hbox{det}}}
\newcommand{\trace}{{\hbox{tr}}}
\newcommand{\sign}{{\hbox{sign}}}
\renewcommand{\arg}{{\hbox{arg}}}
\newcommand{\var}{{\hbox{var}}}
\newcommand{\cov}{{\hbox{cov}}}
\newcommand{\SINR}{{\mathsf SINR}}
\newcommand{\SNR}{{\mathsf SNR}}
\newcommand{\Ei}{{\rm E}_{\rm i}}
\renewcommand{\Re}{{\rm Re}}
\renewcommand{\Im}{{\rm Im}}
\newcommand{\eqdef}{\stackrel{\Delta}{=}}
\newcommand{\defines}{{\,\,\stackrel{\scriptscriptstyle \bigtriangleup}{=}\,\,}}
\newcommand{\<}{\left\langle}
\renewcommand{\>}{\right\rangle}
\newcommand{\herm}{{\mathsf H}}
\newcommand{\trasp}{{\mathsf T}}
\newcommand{\transp}{{\mathsf T}}
\renewcommand{\vec}{{\rm vec}}

\newcommand{\RED}{\color[rgb]{1.00,0.10,0.10}}
\newcommand{\BLUE}{\color[rgb]{0,0,0.90}}
\newcommand{\GREEN}{\color[rgb]{0,0.80,0.20}}

\newcommand{\dt}[1]{{\red #1}}
\newcommand{\ym}[1]{{\cyan #1}}

\newtheorem{thm}{Theorem}%
\newtheorem{cor}{Corollary}
\newtheorem{lem}{Lemma}
\newtheorem{prop}{Proposition}
\newtheorem{rem}{Remark}
\newtheorem{example}{Example}
\newtheorem{defn}{\protect\definitionname}

\providecommand{\definitionname}{Definition}
\providecommand{\lemmaname}{Lemma}
\providecommand{\remarkname}{Remark}
\providecommand{\theoremname}{Theorem}
